Learning Multimodal Bipedal Locomotion and Implicit Transitions: A Versatile Policy Approach

In this paper, we propose a novel framework for synthesizing a single multimodal control policy capable of generating diverse behaviors (or modes) and emergent inherent transition maneuvers for bipedal locomotion. In our method, we first learn efficient latent encodings for each behavior by training an autoencoder from a dataset of rough reference motions. These latent encodings are used as commands to train a multimodal policy through an adaptive sampling of modes and transitions to ensure consistent performance across different behaviors. We validate the policy performance in simulation for various distinct locomotion modes such as walking, leaping, jumping on a block, standing idle, and all possible combinations of inter-mode transitions. Finally, we integrate a task-based planner to rapidly generate open-loop mode plans for the trained multimodal policy to solve high-level tasks like reaching a goal position on a challenging terrain. Complex parkour-like motions by smoothly combining the discrete locomotion modes were generated in 3 min. to traverse tracks with a gap of width 0.45 m, a plateau of height 0.2 m, and a block of height 0.4 m, which are all significant compared to the dimensions of our mini-biped platform.

==> sections/background.tex <==
\section{Background}
\label{sec:back}


% gabe, ethz, osaka's work
% \textbf{Latent Conditioned Policies(LCP)}: For the discovery of diverse skills, the policies are typically modeled as latent/skill conditioned policy given by $\pi(a|s,z)$, where $z \in \mathbb{Z}$, is a latent space of skills or behaviors. Prior work \cite{sharma19} simultaneously discovers predictable skills and a policy where $\pi(a|s,z)$ is optimized such that $z$ is maximally informative about state transitions.
% % and  $q_{\phi}(s'|s,z)$ to approximate the intractable true dynamics, $p(s'|s,z)$ by maximize the likelihood from the samples of $p$. 
% % Recently \cite{OSA202290}, provided an alternate approach by maximizing state and action-based mutual information. 
%  This approach leads to goofy or zombie-like locomotion skills, as there are no explicit regulations on the quality of the motions being learned from scratch. In character animation, \cite{Peng2022} extended the above approach to learn locomotion skills from a library of human motion capture data through simultaneous imitation and skill discovery. \cite{npmp18, football2021} proposes to distill trajectories with a latent bottleneck, where the behaviors observer learns to encode latent representations of the future-state reference trajectories, and the low-level LCP learns to reconstruct the actions given the current state. 
 
% All the above works propose to explore both behavior space and policy space to simultaneously acquire skill representations and a control policy, which leads to the latent skill representations depending either on the current state or a state transition of the agent. Unlike humanoid character control, this can be a major limitation during the absence of morphologically-accurate demonstrations as the state transitions of the targeted agent will then have to significantly vary from that of the experts owing to the difference in dynamics, which is necessarily the case with robot control. 
% Hence we decouple this process, where we first learn efficient latent encoding for all the desired behaviors purely from the demonstration dataset through unsupervised learning and then learn a control policy using those encodings through reinforcement learning. 
% Such a structured pipeline enables us to generate distinct, well-defined behaviours that are user interpretable and thus better suited for application with real robots. 

\textbf{Rough Demonstrations and Waypoints} 
%  While \cite{football2021,Peng2022} show impressive locomotion skills for humanoid character control, learnt from human motion capture data, their dependence on the fidelity of the motion capture data is unclear. That is, the target system (a humanoid character) and the demonstration expert(a human) are morphologically alike, if not exact, with the same form factor and similar dynamics. However, such a rich collection of dynamically-consistent motion capture data is often unavailable for robots of varied form factors and morphologies. 
% A common solution is to generate practical demonstrations from a model-based framework such as TO and use it as a reference for RL policies \cite{bogdanovic22}. This can be restricting as imitation learning is then limited by the performance of the expert (such as TO). Additionally, it is also redundant to perform two full-order optimizations, i.e. TO (model-based) for trajectories followed by RL for a policy to realize those trajectories (model-free). Typically in model-based optimal control, TO is used first to generate dynamically-plausible trajectories based on a rough initial guess as linear interpolation and waypoints \cite{choung21}. These trajectories are then realized through model-based control policies such as MPCs and/or WBCs. In contrast, since RL provides us with a straightforward way to synthesize control policies directly, we ponder the possibility of making the above-mentioned two-stage procedure into a single end-to-end process, i.e, akin to TO, we intend to directly learn a policy to realize locomotion modes from a library of rough demonstrations motions described as linearly interpolated keyframes of the floating base states (i.e. only underactuated 6DOFs of the torso).  Recently \cite{Li2022rough} showcased agile skills learnt through adversarial imitation of rough partial demonstrations that need not be physically feasible. Though the work shows multiple skills, they do so by training different policies for each of the demonstrated behavior. Nonetheless, a key insight is that the physical plausibility of the reference trajectories is not a prerequisite  for the success of RL approaches which further supports our approach. 
 While \cite{football2021, Peng2022} show impressive locomotion skills for humanoid character control learned from human motion capture data, their dependence on the fidelity of the demonstrations is unclear. The target system (a humanoid character) and the demonstration expert (a human) are morphologically alike, with the same form factor and similar dynamics. However, such a rich collection of dynamically-consistent motion capture data is unavailable for robots of varied form factors and morphologies. A common solution is to generate practical demonstrations from a model-based framework, such as TO, for RL policies to imitate \cite{bogdanovic22}, which is redundant as two full-order optimizations are performed concurrently for the same objective.
Additionally, using overspecified rewards and differences in modeling choices can limit RL by TO's performance. Typically, TO generates dynamically-plausible trajectories based on a rough initial guess, such as linear interpolation and waypoints \cite{choung21}, which are then realized by Model Predictive Control (MPC) based controllers. In contrast, since RL provides us with a straightforward way to synthesize control policies, we ponder the possibility of directly learning a policy to realize locomotion modes from a library of rough motion demonstrations. Recently \cite{Li2022rough} showcased agile skills through adversarial imitation of rough partial demonstrations, providing a critical insight that the physical plausibility of the reference trajectories is not vital for the success of RL.


% \textbf{Behavior/Skill Encoding}: For the success of multi-skilled policies, it is essential to have an effective behavior encoding strategy to direct the policy into operating in different locomotion modes. To this end, \cite{sharma19, Vollenweider2022} propose using a user-defined skill distribution where the latent behaviors space is parameterized as one-hot vectors and uniformly sampled during every episode. Such a naive parameterization contains no representational features defining the characteristics of the individual skills, leading to mode aliasing (refer Sec \ref{sec:results}). However, it is well known that the locomotion behaviors for legged systems often exist in a low-dimensional manifold, as compared to the system's full-order state space, and can hence be represented with reduced-order models. Motivated by this, we propose automatically learning characteristic features parameterized as low-dimensional latent vectors, given a repertoire of rough demonstrations.     


% \textbf{Adaptive Sampling}: A major challenge in training multi-skilled policies is to ensure consistent performance across the different skills due to catastrophic forgetting.\cite{Vollenweider2022} tackles this through learning all the skills in parallel,  whereas \cite{Peng2022} proposes to learn a sequence of skills in every episode where a given skill occurs multiple times. However, the above approaches do not consider the inherent bias in the complexity of different skills. For instance, a skill like a backflip may be more complicated to learn than flat-ground walking. Hence, uniformly sampling both these skills in training may not lead to a consistently good performance across each of them as the policy will need more samples to learn a backflip than to walk. Additionally, giving equal exposure to these skills of varied complexity often causes the policy to fall in a local optimum, where it is successful only in a subset of the skills, causing mode collapse. In \cite{body_as19}, a similar difference in complexity across body shape variations was tackled through an adaptive sampling of the body shape parameters to ensure that the challenging variants were encountered more in the training, thus leading to a policy with consistent performance across different body shapes. In accordance with this strategy, we propose a novel adaptive sampling method to ensure consistent performance across different modes and inter-mode transitions that are learnt implicitly.      


\textbf{Adaptive Sampling}: Inconsistency in performance across behaviors of a multi-skilled policy is reflected as mode collapse due to catastrophic forgetting and mode aliasing due to catastrophic remembering. \cite{Vollenweider2022} tackles it by learning all the skills in parallel,  whereas \cite{Peng2022} proposes to learn a sequence of skills in every episode where a given skill occurs multiple times. However, neither of the above considers the inherent bias in the complexity of different skills. For instance, a skill like a backflip may be more complicated than flat-ground walking, thus requiring more samples to master. Additionally, equal exposure to skills of varied complexity often causes the policy to fall in a local optimum, where it is successful only in a subset of the skills, causing mode collapse. \cite{body_as19} tackles a similar variance in complexity across body shape variations through an adaptive sampling of the body shape parameters to ensure the more frequent encountering of challenging variants in training, thereby leading to a consistent policy.


